Mitigating Unhelpfulness in Emotional Support Conversations with Multifaceted AI Feedback

An emotional support conversation system aims to alleviate users' emotional distress and assist them in addressing their challenges. To generate supportive responses, it is critical to consider multiple factors such as empathy, support strategies, and response coherence, as established in prior methods. Nonetheless, previous models occasionally generate unhelpful responses, which intend to provide support but display counterproductive effects. According to psychology and communication theories, poor performance in just one contributing factor might cause a response to be unhelpful. From the model training perspective, since these models have not been exposed to unhelpful responses during their training phase, they are unable to distinguish if the tokens they generate might result in unhelpful responses during inference. To address this issue, we introduce a novel model-agnostic framework named mitigating unhelpfulness with multifaceted AI feedback for emotional support (Muffin). Specifically, Muffin employs a multifaceted AI feedback module to assess the helpfulness of responses generated by a specific model with consideration of multiple factors. Using contrastive learning, it then reduces the likelihood of the model generating unhelpful responses compared to the helpful ones. Experimental results demonstrate that Muffin effectively mitigates the generation of unhelpful responses while slightly increasing response fluency and relevance.

==> tables/tab-human.tex <==
\begin{table}[tb!]
    \centering
    \renewcommand\arraystretch{1.15}
    \begin{tabular}{c|cccc}
    \hline 
    \text{Model} & \text{Ident.} & \text{Comft.} &    \text{Suggt.} & \text{Overall}\\
    \hline
    MultiESC &  &  & &   \\
    Muffin$_{\text{MultiESC}}$ & & & & \\
    \hline
    TransESC &  &  & &   \\
    Muffin$_{\text{TransESC}}$ & & & & \\
    \hline
    KEMI & & &  &  \\
    Muffin$_{\text{KEMI}}$ &  & &  &   \\
    \hline
    \end{tabular}
    \label{tab:human}
    \caption{Human evaluation results.}
\end{table}

